Adversarial Learning Guarantees for Linear Hypotheses and Neural Networks

Adversarial or test time robustness measures the susceptibility of a classifier to perturbations to the test input. While there has been a flurry of recent work on designing defenses against such perturbations, the theory of adversarial robustness is not well understood. In order to make progress on this, we focus on the problem of understanding generalization in adversarial settings, via the lens of Rademacher complexity. We give upper and lower bounds for the adversarial empirical Rademacher complexity of linear hypotheses with adversarial perturbations measured in $l_r$-norm for an arbitrary $r \geq 1$. This generalizes the recent result of [Yin et al.'19] that studies the case of $r = \infty$, and provides a finer analysis of the dependence on the input dimensionality as compared to the recent work of [Khim and Loh'19] on linear hypothesis classes. We then extend our analysis to provide Rademacher complexity lower and upper bounds for a single ReLU unit. Finally, we give adversarial Rademacher complexity bounds for feed-forward neural networks with one hidden layer. Unlike previous works we directly provide bounds on the adversarial Rademacher complexity of the given network, as opposed to a bound on a surrogate. A by-product of our analysis also leads to tighter bounds for the Rademacher complexity of linear hypotheses, for which we give a detailed analysis and present a comparison with existing bounds.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux',0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> shattering.tex <==
	\begin{theorem}
	\label{thm:shattering}
		Let $p<\infty$. Set 
		\[\cG_p^n=\left\{(\bx,y)\to y\sum_{j=1}^n u_j (\bw_j\cdot x)_+: \bu\in S_u, \bW\in S_W\right\}\]
		and
		\[\Pi_\cS^*=\sup_{\substack{\bW\in S_W\\ \bu \in S_u}} \Pi_{\cS}(\bW)\]
			and define	$\mathcal{C}_\cS^*$ to be the total number of possible partitions of $\cS$ that can be obtained as one varies $\bW$. Then
		\[\wt\R^\cS(\cG_p^n)\leq\]
	\end{theorem}
% 	This theorem implies that if $\Pi_\cS^*$ is sub-exponential, then we have a learning guarantee. 
% 	Note that $p<\infty$ is important, this is used in equation (\ref{eq:adv_nn_not_inf}).
	\begin{align}
	&\wt \R_\cS(\cG_p^n)\nonumber\\
	&=\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u}}\frac 1m  \sum_{i=1}^m \sigma_i\inf_{\|\bs\|_r\leq 1} y_i\sum_{j=1}^n u_j(\bw_j\cdot (\bx_i+\e\bs))_+\Bigg]\nonumber\\
	&=\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u}}\frac 1m  \sum_{i=1}^m \sigma_i y_i\sum_{j=1}^n u_j(\bw_j\cdot (\bx_i+\e\bs_i))_+\Bigg]&(\text{definition of }\bs_i)\nonumber\\
	&=\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u}}\frac 1m  \sum_{t=1}^{\Pi_\cS(\bW)}\sum_{i\in \cC_t} \sigma_i y_i\sum_{j=1}^n u_j(\bw_j\cdot (\bx_i+\e\bs_t))_+\Bigg]&(\text{definition of }\cC_t)\nonumber\\
	&\leq\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\Pi_\cS(\bW)\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t} u_j(\bw_j\cdot (\bx_i+\e\bs_t))\Bigg] &\text{(extra supremum)}\nonumber\\
	&\leq\Pi_\cS^*\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t} u_j(\bw_j\cdot (\bx_i+\e\bs_t))\Bigg] &(\text{definition of }\Gamma_\cS^*)\nonumber\\
	&\leq \Pi_\cS^*\left( \E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t} u_j\bw_j\cdot\bx_i\Bigg]+\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t}\e u_j\bw_j\cdot \bs_t))\Bigg] \right) \label{eq:adv_rc_sum}
	\end{align}
	We bound each term in equation (\ref{eq:adv_rc_sum}) separately. For the first term:
	\begin{align}
	& \E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t} u_j\bw_j\cdot\bx_i\Bigg]\nonumber\\
	&=\frac 12  \E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\left|\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t} u_j\bw_j\cdot\bx_i\right|\Bigg]&\text{(sign symmetry)}\nonumber\\
	&=\frac 12  \E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\left|\frac 1m  \sum_{j\in P_t}u_j\bw_j\cdot\sum_{i\in \cC_t} \sigma_i y_i \bx_i\right|\Bigg]&\text{(reordering summations)}\nonumber\\
	&\leq \frac W2  \E_\bsig\Bigg[\sup_{\substack{\bW\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{j\in P_t}|u_j|\left\|\sum_{i\in \cC_t} \sigma_i y_i \bx_i\right\|_{\du p}\Bigg]&\text{(dual norm definition)}\nonumber\\
	&\leq \frac W2  \E_\bsig\Bigg[\sup_{\substack{ \bW, \bu,\cC_t}}\frac 1m  \Lambda\left\|\sum_{i\in \cC_t} \sigma_i y_i \bx_i\right\|_{\du p}\Bigg]&\text{(dual norm definition)}\nonumber\\
	&\leq \frac 1m  \frac {\Lambda W}2  \E_\bsig\Bigg[\sup_{\substack{ \bW, \bu,\cC_t}}\left\|\sum_{i\in \cC_t} \sigma_i \bx_i\right\|_{\du p}\Bigg]&(\sigma_i \text{ distributed like }y_i\sigma_i)\nonumber\\
	&\leq \frac 1m  \frac {\Lambda W}2  \E_\bsig\Bigg[ \sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}}\left\|\sum_{i\in \cC_t} \sigma_i \bx_i\right\|_{\du p} \Bigg]\\
	&\leq \frac 1m  \frac {\Lambda W}2   \sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}}\E_\bsig\Bigg[\left\|\sum_{i\in \cC_t} \sigma_i \bx_i\right\|_{\du p} \Bigg]\\
	&\leq \frac 1m  \frac {\Lambda W}2   \sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}} \sqrt{|C_t|} \max_i \|x_i\|_{\du p}\\
	&\leq \frac 1m  \frac {\Lambda W}2 |\mathcal{C}_{\cS}^*| \sqrt{\Pi_\cS^*} \max_i\|x_i\|_{\du p}.
\end{align}
% 	&=\frac 1m  \frac {\Lambda W}2  \E_\bsig\Bigg[\sup_{\substack{ \bW, \bu,\cC_t}}\sum_{k=1}^d| \sum_{i\in \cC_t}\sigma_i \bx_{ik}|^\du p\Bigg]^\frac 1{\du p}\\
% 	&\leq \frac 1m  \frac {\Lambda W}2  \E_\bsig\Bigg[\sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}}\sum_{k=1}^d| \sum_{i\in \cC_t}\sigma_i \bx_{ik}|^\du p\Bigg]^\frac 1{\du p}\\
% 	&\leq \frac 1m  \frac {\Lambda W}2  \sum_{\mathcal{C}} \sum_{k=1}^d \E_\bsig\Bigg[\sum_{\mathcal{C}} \sum_{k=1}^d| \sum_{i\in \cC_t}\sigma_i \bx_{ik}|^\du p\Bigg]^\frac 1{\du p}\\
	%&\leq \frac W2 \frac 1m  \Lambda\E_\bsig\Bigg[\sup_{\substack{ \bW, \bu,\cC_t}}\sum_{t=1}\left\|\sum_{i\in \cC_t} \sigma_i y_i \bx_i\right\|_{\du p}\Bigg]
%	\end{align}
	Now for the second term in (\ref{eq:adv_rc_sum}):
	\begin{align*}
	&\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{i\in \cC_t} \sigma_i y_i\sum_{j\in P_t}\e u_j\bw_j\cdot \bs_t\Bigg] \nonumber\\
	&=\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m  \sum_{i\in \cC_t} \sigma_i \sum_{j\in P_t}\e u_j\bw_j\cdot \bs_t\Bigg] &(y_i\sigma_i\text{ distributed like }\sigma_i)\nonumber\\
	&=\E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m \sum_{j\in P_t} \e u_j\bw_j\sum_{i\in \cC_t} \sigma_i \cdot \bs_t\Bigg] &\text{(reorder summations)}\nonumber\\
	&\leq \E_\bsig\Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\frac 1m \sum_{j\in P_t} \e |u_j|W\left\|\sum_{i\in \cC_t} \sigma_i \cdot \bs_t\right\|_{\du p}\Bigg]&(\text{dual norm}) \nonumber\\
	&\leq \frac {\epsilon W\Lambda} m \E_\bsig \Bigg[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\left\|\sum_{i\in \cC_t} \sigma_i \cdot \bs_t\right\|_{\du p}\Bigg]&\text{(dual norm)}\nonumber\\
	&\leq \frac {\epsilon W\Lambda} m\sup_{\|\bs_t\|_{\du r} \leq 1}\|\bs_t\|_{\du r} \|\bs_t\|\E_\bsig \Big[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\left|\sum_{i\in \cC_t}\sigma_i\right|\Big]&(\bs_i\text{ constraint})\nonumber\\
	&=\frac {\epsilon W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r})\E_\bsig \Big[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\sum_{i\in \cC_t}\sigma_i\Big]&(\text{lemma \ref{lemma:norm_ratio}})\nonumber\\
	&\leq \frac {\epsilon W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r})\E_\bsig \Big[ \sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}} |\sum_{i\in \cC_t}\sigma_i|\Big]\\
	&\leq \frac {\epsilon W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r})\sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}}\E_\bsig \Big[|\sum_{i\in \cC_t}\sigma_i|\Big]\\
	&\leq \frac {\epsilon W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r})\sum_{\mathcal{C}} \sum_{t=1}^{n_{\mathcal{C}}} \sqrt{|C_t|}\\
	&\leq \frac {\epsilon W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r}) |\mathcal{C}_{\cS}^*|\sqrt{\Pi_\cS^*}.
% 	&= \frac {W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r})\E_\bsig \Big[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\sup_{\tau\in{\pm1}}\sum_{i\in \cC_t}\tau\sigma_i\Big]\nonumber\\
% 	&=\frac {W\Lambda} m\max(1,d^{1-\frac 1p -\frac 1r})\E_\bsig \Big[\sup_{\substack{\bW\in S_W\\ \bu \in S_u\\ \cC_t}}\sup_{\tau\in{\pm1}}\sum_{i=1}^n\tau I_{\bx_i\in \cC_t}\sigma_i\Big]&(I\text{ indicator function})\nonumber\\
% 	&\leq \frac {W\lambda \sqrt{4 m\log\Pi_\cS^*}} m=\frac {2W\lambda \sqrt{\log\Pi_\cS^*}} {\sqrt m}
	\end{align*}
% 	Where the last line follows from Massart's lemma we have $2\Pi^*_\cS$ vectors because of the sign $\tau$.
